Learning Lane Graphs from Aerial Imagery Using Transformers

The robust and safe operation of automated vehicles underscores the critical need for detailed and accurate topological maps. At the heart of this requirement is the construction of lane graphs, which provide essential information on lane connectivity, vital for navigating complex urban environments autonomously. While transformer-based models have been effective in creating map topologies from vehicle-mounted sensor data, their potential for generating such graphs from aerial imagery remains untapped. This work introduces a novel approach to generating successor lane graphs from aerial imagery, utilizing the advanced capabilities of transformer models. We frame successor lane graphs as a collection of maximal length paths and predict them using a Detection Transformer (DETR) architecture. We demonstrate the efficacy of our method through extensive experiments on the diverse and large-scale UrbanLaneGraph dataset, illustrating its accuracy in generating successor lane graphs and highlighting its potential for enhancing autonomous vehicle navigation in complex environments.

==> sections/2_related_work.tex <==
\section{Related Work}


==> tables/analysis.tex <==
    \begin{table}
        \centering
        \caption{Analysis of the different model behaviors. }
        \label{tab:analysis}
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|YYY}
          \toprule
            Model & \# Object Interactions & Distance Travelled & Infeasible Actions\\
          \midrule
            Random               & 7.0 & 42.4 & --\\
            Greedy               & 8.6 & 24.7 & --\\
            Random w/ door-prior & 9.3 & 25.7 & --\\
            Greedy w/ door-prior & 9.0 & 25.0 & --\\
            \midrule
            ESC                  & 5.8 & 28.2 & --\\
            HIMOS                & 5.3 & 43.2 & --\\
            % SSG?&& \\
            \midrule
            Unstructured LLM     & 3.9 & 19.2 & 0.51 \\
            \ours{}              & 4.2 & 19.2 & 0.35 \\
          \bottomrule
        \end{tabularx}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Average over all episodes (including failures). Distance travelled in meters. Infeasible Actions is the average number of steps in which the LLM produces an action that could not be executed.
         \end{tablenotes}
       \end{threeparttable}
    \end{table}

==> tables/compute_analysis.tex <==
\begin{table}
    \centering
    \caption{Evaluation of the average time used by each system component.}
    \label{tab:compute}
    \begin{threeparttable}
    \begin{tabularx}{\linewidth}{l|YY}
      \toprule
        Component & Total time (\unit{\second}) & Share (\%) \\
      \midrule
        \textit{Total}                    & 457$^*$& 100$^*$\\
        \midrule
        \textit{Low-level Execution}      & 250$^*$& \phantom{0}55$^*$\\
        Navigation                        & 139$^*$& \phantom{0}30$^*$\\
        Manipulation                      & 111$^*$& \phantom{0}24$^*$\\
        \midrule
        \textit{High-level Reasoning}     & 207$^*$& \phantom{0}45$^*$\\
        Scene Graph Construction          & -   & $\dag$\\
        Room Classification               & -   & $\dag$\\
        LLM Reasoning                     & -   & $\dag$\\
      \bottomrule
    \end{tabularx}
    \begin{tablenotes}[para,flushleft]
       \footnotesize      
       $^*$Average over three episodes of the fuzzy-search real world experiments.\\$\dag$Average over 175 simulation episodes in iGibson.
     \end{tablenotes}
   \end{threeparttable}
\end{table}

==> tables/distance_encoding.tex <==
    \begin{table}
        \centering
        \caption{Mapping of distances to natural language.}
        \label{tab:distance_encoding}
        \begin{tabularx}{\linewidth}{Y|Y}
          \toprule
            $\le$ Distance & Encoding \\
          \midrule
            \phantom{0}3.0 & very close\\
            10.0 & near \\
            20.0 & far \\
            \phantom{0}$\infty$ & distant\\
          \bottomrule
        \end{tabularx}
    \end{table}

==> tables/fuzzy_search.tex <==
    \begin{table*}
        \scriptsize
        \centering
        \caption{Results on the fuzzy search tasks in the Real World. }
        \label{tab:fuzzy_search}%
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|cY}
          \toprule
            Task & Success & Reasoning \\
          \midrule
            I am hungry. Find me something for breakfast.      & \cmark & Found cereals, toast, coffee. Then opened fridge to look for milk or eggs. Found milk in the fridge and decided these are sufficient items.\\
            Find me something to wash my hands.                & \cmark & Searched kitchen for a sink. When not finding one, searches for storage room or bathroom until it finds the sink in the bathroom.\\
            I feel sleepy. Find me something to wake up.       & \cmark & The teapot is associated with tea that contains caffeine and can help someone wake up.\\
            Find things to set the kitchen table.              & \cmark & Explored kitchen, opening cabinets. Found knife, glasses, plates. Continued to look for forks or spoons. When not finding them, called done. (No forks or spoons existed).\\
            Find me the book in the living room.               & \cmark & Explored until finding living room, then opened cabinet looking for book, found it inside. \\
          \midrule
            Pour me a glass of milk.                           & \cmark & Finds milk in fridge, glass on table. Navigates between the two, assuming to transport the last object. Then terminates, reasoning that it has found and navigated to both.\\
            Turn on the oven.                                  & \cmark & Finds the oven and calls done(): "Turning on oven is implied as completion of the task".\\
            What's the time?                                   & \cmark & Finds the clock and calls done(): "The clock is the object that will provide the time".\\
          \bottomrule
        \end{tabularx}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Top: fuzzy search queries. Bottom: infeasible task queries. Success in these tasks is evaluated by human judgment as a reasonable response. The reasoning has been qualitatively paraphrased for brevity.
         \end{tablenotes}
       \end{threeparttable}
       \vspace{-0.3cm}
    \end{table*}


==> tables/prompt_ablations.tex <==
    \begin{table}
        \scriptsize
        \setlength{\tabcolsep}{4pt}
        \centering
        \caption{Prompt Ablations}\label{tab:prompt_ablations}
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|ccc|ccc}
          \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{SR} & \multirow{2}{*}{SPL} & \multirow{2}{*}{AUC-E} & Object & Distance & Infeasible\\
             &  &  &  & Interactions & Traveled & Actions\\
            \midrule
            Unstructured LLM (w/ action history and frontiers)       & 81.4 & 55.0 & 72.8 & \textbf{3.9} & \textbf{\underline{19.2}} & \underline{0.51} \\
            \midrule
            Structured Room-Object encoding w/o action-history, w/o frontiers & 76.0 & 55.8 & 69.6 & 3.9 & 13.7 & 0.85 \\
            Structured Room-Object encoding + coarse action-history, w/o frontiers & 79.4 & 54.9 & 72.4 & 4.2 & 15.5 & 0.94 \\
            Structured Room-Object encoding + coarse action-history + frontiers & \textbf{97.1} & \textbf{63.0} & \textbf{86.6} & \textbf{3.8} & 17.8 & \textbf{0.28} \\
            Structured Room-Object encoding + action-history, w/o frontiers & 79.4 & 55.0 & 72.2 & 4.3 & 15.6 & 0.91 \\
            Structured Room-Object encoding + frontiers, w/o action-history & 94.9 & 63.0 & 84.1 & 3.6 & 17.1 & 0.26 \\
            \ours{} w/o distances and nearby objects & 97.1 & 61.5 & 86.4 & 3.8 & 18.9 & 0.24 \\
            \midrule
            \ours{} (ours)               & \underline{92.6} & \underline{59.9} & \underline{82.5} & \underline{4.2} & \textbf{\underline{19.2}} & \underline{0.35} \\
            \midrule
            \ours{} w/o max. history length?\\
          \bottomrule
        \end{tabularx}
        \vspace{-0.cm}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Best and second best highlighted in bold and underline. Object interactions, distance travelled and infeasible actions averaged over all episodes - including early terminated failures. Infeasible Actions: average number of steps the LLM produced an action that could not be executed, resulting in re-planning with continued conversation (cf. Sec. IV-C.4).
         \end{tablenotes}
       \end{threeparttable}
       \vspace{-0.3cm}
    \end{table}

==> tables/real_world_experiments.tex <==
    \begin{table}
    \vspace{-0.2cm}
        \centering
        \caption{Interactive Object Search Results in the Real World }
        \vspace{-0.2cm}
        \label{tab:real_world_experiments}%
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|YYYYY}
          \toprule
            \multirow{2}{*}{Model} & Success & Navig & Manip & Distance & Object \\
                                   & Rate & Fails & Fails & Traveled & Interact. \\
          \midrule
            ESC-Inter. & 80\% & 2 & 0 & 33.9 & 3.5 \\
            \ours{}    & 80\% & 1 & 1 & \textbf{17.9} & \textbf{2.2} \\
          \bottomrule
        \end{tabularx}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Dist. travelled is the average distance travelled per episode in meters. Object interactions are the average number of object interactions per episode.
         \end{tablenotes}
       \end{threeparttable}
    %\vspace{-0.3cm}
    \end{table}


==> tables/scene_graph_evaluation.tex <==
\begin{table}
    \centering
    \caption{Scene Graph Evaluation}
    \label{tab:graph_eval}
    \begin{tabularx}{\linewidth}{lc|cc}
      \toprule
        Environment & Open-Set & Purity $G_{\mathcal{V}}^{R}$ & Room Category Accuracy \\
      \midrule
         iGibson & $\times$ & 0.609 & 0.276 \\
         Real-World & $\checkmark$ &- & 0.901 \\
      \bottomrule
    \end{tabularx}
\end{table}

==> tables/sim_experiments.tex <==
% \begin{figure*}
%   \footnotesize
%   \begin{minipage}[H]{.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/raw/auc_curve.png}%
%     % \caption
%     %   {%
%     %     Efficiency curve in simulation%
%     %     \label{fig:duck}%
%     %   }%
%   \end{minipage}\hfill
%   \begin{minipage}[H]{.52\linewidth}
%     \centering
    \begin{table}
        \scriptsize
        \setlength{\tabcolsep}{4pt}
        \centering
        \caption{Interactive Object Search Results in Simulation}\label{tab:sim_experiments}
        \begin{threeparttable}
        \begin{tabularx}{\linewidth}{l|ccc|ccc}
          \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{SR} & \multirow{2}{*}{SPL} & \multirow{2}{*}{AUC-E} & Object & Distance & Infeasible\\
             &  &  &  & Interactions & Traveled & Actions\\
          % \midrule
          % Non-interactive task\\
          % \midrule
          % Random                   & 90.6 & \textbf{99.4} & 61.3\\
          % Greedy                   & 90.5 & 98.9 & 64.8\\
          % ESC                      & \textbf{91.0} & 98.3 & \textbf{66.6}\\
          % HIMOS                    & 81.1 & 97.1 & 42.9 \\
          % Unstructured LLM         & 69.6 & 75.3 & 54.3 \\
          % \ours{}                  & 89.5 & 96.6 & 66.2\\
          % \midrule
          % \midrule
          % %   Heuristic w/o Scene-underst. & \xmark & \cmark & \\
          % Interactive task\\
          \midrule
          % \midrule
            Random                 & 88.8 & 45.8 & 71.8 & 7.0 & 42.4 & --\\
            Greedy                 & 81.1 & 47.2 & 68.8 & 8.6 & 24.7 & --\\
            % Rand. w/ door-prior   & 80.6 & 47.5 & 68.5 & 9.3 & 25.7 & --\\
            % Greedy w/ door-prior   & 80.0 & 47.8 & 68.5 & 9.0 & 25.0 & --\\
            \midrule
            ESC-Interactive        & 90.3 & 52.0 & \underline{77.5}& 5.8 & 28.2 & --\\
            HIMOS                  & \textbf{93.1} & 47.5 & 75.7& 5.3 & 43.2 & --\\
            % SSG?                 && \\
            \midrule
            Unstructured LLM       & 81.4 & \underline{55.0} & 72.8 & \textbf{3.9} & \textbf{\underline{19.2}} & \underline{0.51} \\
            % Ours w/o scene-graph?  & \xmark & \cmark & & \\
            \ours{} (ours)               & \underline{92.6} & \textbf{59.9} & \textbf{82.5} & \underline{4.2} & \textbf{\underline{19.2}} & \textbf{0.35} \\
          \bottomrule
        \end{tabularx}
        \vspace{-0.cm}
        \begin{tablenotes}[para,flushleft]
           \footnotesize      
           Notes: Best and second best highlighted in bold and underline. Object interactions, distance travelled and infeasible actions averaged over all episodes - including early terminated failures. Infeasible Actions: average number of steps the LLM produced an action that could not be executed, resulting in re-planning with continued conversation (cf. Sec. IV-C.4).
         \end{tablenotes}
       \end{threeparttable}
       \vspace{-0.3cm}
    \end{table}
%   \end{minipage}
%   \caption{Interactive Object Search Results in Simulation. Left: efficiency curve, right: AUC-E: area under the efficiency curve, SR: success rate, SPL: success weighted by path length.}
%   \label{tab:sim_experiments}
% \end{figure*}





